Dynamics, radiation and overall energy budget of earthquake rupture with coseismic off-fault damage

Earthquake ruptures dynamically activate coseismic off-fault damage around fault cores. Systematic field observation efforts have shown the distribution of off-fault damage around main faults, while numerical modeling using elastic-plastic off-fault material models has demonstrated the evolution of coseismic off-fault damage during earthquake ruptures. Laboratory scale micro-earthquake experiments have pointed out the enhanced high-frequency radiation due to the coseismic off-fault damage. However, the detailed off-fault fracturing mechanisms, subsequent radiation and its contribution to the overall energy budget remain to be fully understood because of limitations of current observational techniques and model formulations. Here, we constructed a new physics-based dynamic earthquake rupture modeling framework, based on the combined finite-discrete element method (FDEM), to investigate the fundamental mechanisms of coseismic off-fault damage, and its effect on the rupture dynamics, the radiation and the overall energy budget. We conducted a 2-D systematic case study with depth and showed the mechanisms of dynamic activation of the coseismic off-fault damage. We found the decrease in rupture velocity and the enhanced high-frequency radiation in near-field due to the coseismic off-fault damage. We then evaluated the overall energy budget, which shows a significant contribution of the coseismic off-fault damage to the overall energy budget even at depth, where the damage zone width becomes narrower. The present numerical framework for the dynamic earthquake rupture modeling thus provides the insight into the earthquake rupture dynamics with the coseismic off-fault damage.

==> abstractarxive.tex <==
% !TEX root = ../Okuboetal.tex
\abstract{Earthquake ruptures dynamically activate coseismic off-fault damage around fault cores. Systematic field observation efforts have shown the distribution of off-fault damage around main faults, while numerical modeling using elastic-plastic off-fault material models has demonstrated the evolution of coseismic off-fault damage during earthquake ruptures. Laboratory scale micro-earthquake experiments have pointed out the enhanced high-frequency radiation due to the coseismic off-fault damage. However, the detailed off-fault fracturing mechanisms, subsequent radiation and its contribution to the overall energy budget remain to be fully understood because of limitations of current observational techniques and model formulations. Here, we constructed a new physics-based dynamic earthquake rupture modeling framework, based on the combined finite-discrete element method (FDEM), to investigate the fundamental mechanisms of coseismic off-fault damage, and its effect on the rupture dynamics, the radiation and the overall energy budget. We conducted a 2-D systematic case study with depth and showed the mechanisms of dynamic activation of the coseismic off-fault damage. We found the decrease in rupture velocity and the enhanced high-frequency radiation in near-field due to the coseismic off-fault damage. We then evaluated the overall energy budget, which shows a significant contribution of the coseismic off-fault damage to the overall energy budget even at depth, where the damage zone width becomes narrower. The present numerical framework for the dynamic earthquake rupture modeling thus provides the insight into the earthquake rupture dynamics with the coseismic off-fault damage.}


==> sections/abstract.tex <==
% !TEX root = ../Okuboetal.tex
\begin{abstract} Earthquake ruptures dynamically activate coseismic off-fault damage around fault cores. Systematic field observation efforts have shown the distribution of off-fault damage around main faults, while numerical modeling using elastic-plastic off-fault material models has demonstrated the evolution of coseismic off-fault damage during earthquake ruptures. Laboratory scale micro-earthquake experiments have pointed out the enhanced high-frequency radiation due to the coseismic off-fault damage. However, the detailed off-fault fracturing mechanisms, subsequent radiation and its contribution to the overall energy budget remain to be fully understood because of limitations of current observational techniques and model formulations. Here, we constructed a new physics-based dynamic earthquake rupture modeling framework, based on the combined finite-discrete element method (FDEM), to investigate the fundamental mechanisms of coseismic off-fault damage, and its effect on the rupture dynamics, the radiation and the overall energy budget. We conducted a 2-D systematic case study with depth and showed the mechanisms of dynamic activation of the coseismic off-fault damage. We found the decrease in rupture velocity and the enhanced high-frequency radiation in near-field due to the coseismic off-fault damage. We then evaluated the overall energy budget, which shows a significant contribution of the coseismic off-fault damage to the overall energy budget even at depth, where the damage zone width becomes narrower. The present numerical framework for the dynamic earthquake rupture modeling thus provides the insight into the earthquake rupture dynamics with the coseismic off-fault damage.
\end{abstract}

